Wav2Gloss: Generating Interlinear Glossed Text from Speech

Thousands of the world's languages are in danger of extinction--a tremendous threat to cultural identities and human language diversity. Interlinear Glossed Text (IGT) is a form of linguistic annotation that can support documentation and resource creation for these languages' communities. IGT typically consists of (1) transcriptions, (2) morphological segmentation, (3) glosses, and (4) free translations to a majority language. We propose Wav2Gloss: a task in which these four annotation components are extracted automatically from speech, and introduce the first dataset to this end, Fieldwork: a corpus of speech with all these annotations, derived from the work of field linguists, covering 37 languages, with standard formatting, and train/dev/test splits. We provide various baselines to lay the groundwork for future research on IGT generation from speech, such as end-to-end versus cascaded, monolingual versus multilingual, and single-task versus multi-task approaches.

==> chapters/06-future-work.tex <==
\section{Future Work}

\subsection{Normalization}
Normalization of IGT labels can enable corpus studies of linguistic phenomena across a diverse set of languages. However, the process is labor intensive, as previous research \citep{ListSimsForkel2021} and we ourselves have observed. Normalization is an important next step for \dataset{} to improve both the usefulness and quality of the dataset.

\subsection{Expansion to other sources}
People familiar with language resource archives will perhaps note the conspicuous absence of three of the largest archives of field linguistics -- TLA, ELAR, and PARADISEC. We forego these archives for this work mostly due to time and resource constraints, and will hopefully include them in the future. The challenges shared by the expansion to the three archives are mostly due to their size and the work required to filter, extract, and obtain rights for the data. Most of this work will have to be done on a language-by-language basis to ensure quality.


